Improving Autoregressive Visual Generation with Cluster-Oriented Token Prediction

Employing LLMs for visual generation has recently become a research focus. However, the existing methods primarily transfer the LLM architecture to visual generation but rarely investigate the fundamental differences between language and vision. This oversight may lead to suboptimal utilization of visual generation capabilities within the LLM framework. In this paper, we explore the characteristics of visual embedding space under the LLM framework and discover that the correlation between visual embeddings can help achieve more stable and robust generation results. We present IAR, an Improved AutoRegressive Visual Generation Method that enhances the training efficiency and generation quality of LLM-based visual generation models. Firstly, we propose a Codebook Rearrangement strategy that uses balanced k-means clustering algorithm to rearrange the visual codebook into clusters, ensuring high similarity among visual features within each cluster. Leveraging the rearranged codebook, we propose a Cluster-oriented Cross-entropy Loss that guides the model to correctly predict the cluster where the token is located. This approach ensures that even if the model predicts the wrong token index, there is a high probability the predicted token is located in the correct cluster, which significantly enhances the generation quality and robustness. Extensive experiments demonstrate that our method consistently enhances the model training efficiency and performance from 100M to 1.4B, reducing the training time by half while achieving the same FID. Additionally, our approach can be applied to various LLM-based visual generation models and adheres to the scaling law, providing a promising direction for future research in LLM-based visual generation. The code is available at: https://github.com/sjtuplayer/IAR.

==> sec/0_abstract.tex <==
\begin{abstract}

% Employing LLMs for visual generation has recently become a research focus. However, the existing methods primarily transfer the LLM architecture to visual generation but rarely investigate the fundamental differences between language and vision. This oversight may lead to suboptimal utilization of visual generation capabilities within the LLM framework. In this paper, we explore the characteristics of visual embedding space under the LLM framework and discover that the correlation between visual embeddings can help achieve more stable and robust generation results. We present IAR, an Improved AutoRegressive Visual Generation Method that enhances the training efficiency and generation quality of LLM-based visual generation models. Firstly, we propose a Codebook Rearrangement strategy that uses balanced k-means clustering algorithm to rearrange the visual codebook into clusters, ensuring high similarity among visual features within each cluster. Leveraging the rearranged codebook, we propose a Cluster-oriented Cross-entropy Loss that guides the model to correctly predict the cluster where the token is located. This approach ensures that even if the model predicts the wrong token index, there is a high probability the predicted token is located in the correct cluster, which significantly enhances the generation quality and robustness. Extensive experiments demonstrate that our method consistently enhances the model training efficiency and performance from 300M to 1.5B, reducing the training time by half while achieving the same FID. Additionally, our approach can be applied to various LLM-based visual generation models and adheres to the scaling law, providing a promising direction for future research in LLM-based visual generation.



\yr{Employing LLMs for visual generation has recently become a research focus.}
However, \yr{the existing} methods primarily \yr{transfer} the LLM architecture to \yr{visual} generation \yr{but rarely} investigat\yr{e} the \yr{fundamental} differences between language and vision. This oversight may lead to suboptimal utilization of visual generation capabilities within the LLM framework.
In this paper, we explore \yr{the characteristics of} visual \yr{embedding space} under the LLM framework and discover that the correlation between visual embeddings can help achieve more stable and robust generation results. 
\yr{We present \hut{\textbf{IAR}, an \textbf{I}mproved \textbf{A}uto\textbf{R}egressive Visual Generation Method that enhances} the training efficiency and generation quality of LLM-based visual generation models. Firstly,}
we propose a \yr{Codebook Rearrangement strategy that uses} balanced k-means clustering algorithm to rearrange the visual codebook \yr{into clusters}, ensuring high similarity among visual features within each cluster. 
Leveraging the rearranged codebook, we \yr{propose} a Cluster-oriented Cross-entropy Loss that \yr{guides} the model \yr{to correctly predict the cluster where the target token is located.} %locate the cluster index. 
This approach ensures that even if the model predicts the wrong token index, there is a high probability the predicted token is located in the correct cluster, which significantly enhances the \yr{generation} quality and robustness. %of the generated images. 
\yr{Extensive} experiments demonstrate that our IAR \yr{consistently enhances the model training efficiency and performance from 100M to 1.4B, reducing the training time by half while achieving the same FID.}
%can almost double the training efficiency and achieve better generation quality under the same number of epochs. 
Additionally, IAR can be applied to \yr{various} LLM-based visual generation model\yr{s} and adheres to the scaling law, providing a \yr{promising} direction for future research in LLM-based visual generation. \car{The code is available at: \href{https://github.com/sjtuplayer/IAR}{\textcolor{magenta}{https://github.com/sjtuplayer/IAR}}}.



\end{abstract}
